Sample Efficient Actor-Critic with Experience Replay

This paper presents an actor-critic deep reinforcement learning agent with experience replay that is stable, sample efficient, and performs remarkably well on challenging environments, including the discrete 57-game Atari domain and several continuous control problems. To achieve this, the paper introduces several innovations, including truncated importance sampling with bias correction, stochastic dueling network architectures, and a new trust region policy optimization method.

==> sections/discussion.tex <==
%!TEX root = ../replay.tex


\section{Theoretical Analysis}
\label{sec:analysis}

Retrace is a very recent development in reinforcement learning. In fact, this work is the first to consider Retrace in the policy gradients setting. For this reason, and given the core role that Retrace plays in ACER, it is valuable to shed more light on this technique. In this section, we will prove that Retrace can be interpreted as an application of the importance weight truncation and bias correction trick advanced in this paper. 

Consider the recursive definition of the $\lambda$-returns:
\be
R^{\lambda}_{t} = r_t + (1-\lambda)\gamma V^{\pi}(x_{t+1}) + \lambda \gamma  \rho_{t+1} R^{\lambda}_{t+1}.
\label{eqn:lamrtns}
\ee
Taking expectations of the above expression under the behavior policy, we obtain:
\be
Q^{\pi}(x_t, a_t) = \mathbb{E}_{x_{t+1}a_{t+1}} \left[ r_t + (1-\lambda)\gamma V^{\pi}(x_{t+1}) + 
\lambda \gamma 
\rho_{t+1} Q^{\pi}(x_{t+1}, a_{t+1})\right].
\label{eqn:qrtns}
\ee
\todo{This step is not well justified: $\E[ \rho_{t+1} R^{\lambda}_{t+1}] \neq \E[ \rho_{t+1} \E[R^{\lambda}_{t+1}]]$.}
We can now apply the importance weight truncation with bias correction (tbc) trick to $Q^{\pi}(x_{t+1}, a_{t+1})$  to obtain: 
\bea
Q^{\mbox{\small tbc}}(x_t, a_t) = \mathbb{E}_{x_{t+1}a_{t+1}} \left[  r_t + (1-\lambda)\gamma V(x_{t+1})  \hspace{-3mm}\right. &+&  \hspace{-3mm} 
\gamma \lambda \min\left\{c, \rho_{t+1} \right\}Q^{\mbox{\small tbc}}(x_{t+1}, a_{t+1})  \nonumber \\
 \hspace{-3mm} &+& \left. \hspace{-3mm} \gamma \lambda  \hspace{-1mm} \int  \hspace{-1mm} \left[1\hspace{-.5mm}  - \hspace{-.5mm} \frac{c}{\rho_{t+1}(a)} \right]_+
  \hspace{-3mm} Q(x_{t+1}, a) \pi(a|x_{t+1})da   \hspace{-.5mm}  \right] \hspace{-1mm} .
\label{eqn:qcomp}
\eea
\todo{What is $Q$ here?}

\begin{proposition}
$Q^{\mbox{\small tbc}}$ is a contraction. \todo{A function $Q^{\mbox{\small tbc}}$ is not a contraction. An operator can be a contraction.} Specifically, for $0 \leq C_{t+1} \leq 1$ and for all $x_t$ and $a_t$, we have:
\bea
\left|Q^{\mbox{\small tbc}}(x_t, a_t) - Q^{\pi}(x_t, a_t)\right|  
		 &\leq&
		 \gamma \sup_{x_{t+1}} \biggl[  C_{t+1} \sup_{a}|Q^{\mbox{\small tbc}}(x_{t+1}, a) - Q^{\pi}(x_{t+1}, a)| + \nonumber \\
		& &  (1-C_{t+1})\sup_{a}\left|(Q(x_{t+1}, a) - Q^{\pi}(x_{t+1}, a)  \right| \biggl] .
\eea
\end{proposition}


\begin{proposition}
Retrace is equal to $Q^{\mbox{\small tbc}}$ in expectation with $\lambda = 1$. Specifically,
\begin{align}
	\mathbb{E}_{a_{t+1}}[Q^{\mbox{\small tbc}}(x_t, a_t)] &= 
	\mathbb{E}_{a_{t+1}}\left[r_t + 
		\gamma \lambda \bar{\rho}_{t+1} (Q^{\mbox{\small tbc}}(x_{t+1}, a_{t+1})-Q(x_{t+1}, a_{t+1}) + \gamma V(x_{t+1}) \right].
	\label{eqn:qreta}
\end{align}
\end{proposition}

The above propositions not only confirm that retrace is a contraction, but also show a new way of deriving retrace.
\todo{Retrace is defined by a specific choice of the trace cutting coefficients $c=\lambda\min(1,\mu/\pi)$. Other choices are possible with similar guarantees. This choice has been made for several reasons but this is definitively not the optimal solution in any sense! So there is no principle way of deriving Retrace. Retrace is just a choice.}
Please refer to Appendix~\ref{sec:retraceAsTrick} of the proofs for the above propositions.


\section{Concluding Remarks}
\label{sec:conclusion}

We have proposed a beautiful thing. People love it because it wins. Wins. It's gonna be great. \todo{Agreed!}



% 
% We have shown that the proposed off-policy A3C algorithm outperforms on-policy A3C with a $Q$ baseline in terms of sample complexity. The new algorithm is both stable and efficient over a diverse set of tests, including 57 Atari games and partially-observed \textsc{Labyrinth} tasks.
% 
% It should be possible to further improve the algorithm by adopting dueling architectures \cite{Wang:2016} and prioritized replay \cite{Schaul:2015}. The deployment of the algorithm for continuous control tasks is another potentially fruitful research direction.
% 
% The introduction of episodic memory opens up many avenues for interesting future research. 
% For instance, the architecture described thus far uses a local episodic memory for each thread.
% While this approach dramatically improved data-efficiency, allowing threads to exchange (part of) their memory could lead to further improvements.
% 
% For a taste of this, we implemented experience sharing between threads. More concretely, every time a thread terminates an episode, it can write (part of) the episodic experience to a common pool of experiences from where other threads can pick episodes to augment their memory. 
% % Preliminary experiments revealed that simply adding this functionality while writing all the episodes into the pool blindly yielded strictly comparable results to our previous implementation. 
% % It had been shown~\cite{Schaul:2015} how prioritized sampling could drastically improve the performance of learning algorithms. 
% %Instead of writing every episode to the shared memory, we do it with an episode-dependent probability $p$. 
% In our {prioritized experience sharing} approach, the threads only share
% episodes with a high average absolute temporal-difference error. We can think of this as threads story-telling or blogging interesting experiences, which other threads can consume.
% 
% Experiments on a few Atari games (see Figure~\ref{fig:prioritization}) reveal that the use of prioritized experience sharing can dramatically speed up learning particularly in situations where the A3CR algorithm is stuck in poor local minima. The design of more structured episodic memory architectures for replay appears to be one of the most promising future research endeavours. 
% % However, it also diminishes performances on other games. A more detailed study will be needed in order to assess how to optimize the benefits of prioritized experience sharing across all the games (possibly by combining it with prioritized sampling and/or importance sampling)
% 
% % We have so far introduced a practical off-policy actor critic algorithm. 
% % We believe that this is an important first step that opens doors to a number future research directions. 
% % One such direction is to extend prioritize experience replay~\cite{Schaul:2015} to the
% % actor critic setting.
% % In a pilot study, we study a simple implementation of 
% % we maintained a shared pool of episodes that have high average 
% % absoluate TD-errors. 


